A Simple and Approximately Optimal Mechanism for an Additive Buyer

We consider a monopolist seller with $n$ heterogeneous items, facing a single buyer. The buyer has a value for each item drawn independently according to (non-identical) distributions, and her value for a set of items is additive. The seller aims to maximize his revenue. We suggest using the a-priori better of two simple pricing methods: selling the items separately, each at its optimal price, and bundling together, in which the entire set of items is sold as one bundle at its optimal price. We show that for any distribution, this mechanism achieves a constant-factor approximation to the optimal revenue. Beyond its simplicity, this is the first computationally tractable mechanism to obtain a constant-factor approximation for this multi-parameter problem. We additionally discuss extensions to multiple buyers and to valuations that are correlated across items.

==> PRev.tex <==
\section{Many i.i.d. bidders: Max\{SRev, BRev\} vs. PRev}
In this section, we show that for any number of i.i.d. bidders, $Max\{SRev, BRev\} = \Omega(PRev)$. The techniques are drastically different than those employed in previous sections, so we give a brief outline of our approach below.

First, we show that for i.i.d. bidders, it suffices to consider \emph{pricing mechanisms} rather than second price auctions. A pricing mechanism simply sets a price on the item (or bundle of items) being sold, and awards it to any bidder willing to pay that price (breaking ties arbitrarily). In other words, a pricing mechanism differs from an auction with reserve in that it breaks ties arbitrarily instead of extracting extra revenue from the competition among those willing to pay. We first show that the extra revenue coming from competition does not account for more than a constant factor, so we may restrict attention to pricing mechanisms, which greatly simplifies the analysis. We use the terms SPricingRev, BPricingRev, and PPricingRev to discuss the optimal revenue obtainable by the pricing mechanism counterparts to SRev, BRev, and PRev.

From here, we denote by $(S,p)$ the pricing mechanism that sells the subset of goods $S$ at price $p$ and consider two operations on pricing mechanisms. BUNDLE takes several disjoint schemes $(S_1,p_1),\ldots,(S_k,p_k)$ (by disjoint we mean that $S_i \cap S_j = \emptyset$) and sets a single price $p$ on the entire bundle $S = \cup_i S_i$. SHATTER takes a single scheme $(S,p)$ and sets a price $p_i$ on each item $i \in S$. We then want to understand when the revenue of the original schemes is preserved under BUNDLE and SHATTER. 

We will show that whenever each $(S_i,p_i)$ is such that a single consumer is willing to purchase $S_i$ at price $p_i$ with probability at least $c_1$, then the revenue obtained by BUNDLE is at least $c_2\sum_{i=1}^k BPricingRev(S_i,p_i)$. We will also show that whenever $(S,p)$ is such that a single consumer is willing to purchase $S$ at price $c_3p$ with probability at most $c_1$, then the revenue obtained by SHATTER is at least $c_4 BPricingRev(S,p)$.

This immediately yields a proof that $\max\{SPricingRev,BPricingRev\} \geq cPPricingRev$: Start with an arbitrary partition pricing mechanism and look at each partition. For each subset in the partition, either selling the subset at $c_3$ times the optimal price sells with probability at least $c_1$, or it doesn't. Run BUNDLE on the partitions where it does (after multiplying all prices by $c_3$), and SHATTER on the partitions where it doesn't. One of these collections of subsets accounts for at least half of PPricingRev, and both BUNDLE and SHATTER perform well on the partitions to which they're applied. As BUNDLE outputs a price on just the grand bundle, and SHATTER outputs a price on every item separately, we see that either SPricingRev or BPricingRev performs well compared to PPricingRev.

\subsection{Pricing Mechanisms}
In this section we show that it suffices to consider pricing mechanisms, up to losing a constant factor in our guarantee. In the following section, when we write $BRev_p$, we mean that $p$ is the reserve used by the mechanism. Similarly, when we write $BPricingRev_p$, we mean that the price used is $p$. 
\begin{lemma}\label{lem:split}
$BRev_p \leq BPricingRev_p + BRev_0$.
\end{lemma}

\begin{proof}
We will actually prove the stronger statement that this bound holds on a per-profile basis. On any possible bid profile, either zero, one, or more than one bidders have value larger than $p$. If zero bidders have value larger than $p$, then the contribution to $BRev_p$ is $0$, so the bound holds. If one bidder has value larger than $p$, then the contribution to $BRev_p$ is $p$, and so is the contribution to $BPricingRev_p$, so the bound holds. Finally, if multiple bidders have value larger than $p$, then the contribution to $BRev_p$ is equal to the second highest bid, and so is the contribution to $BRev_0$, so the bound holds.
\end{proof}

\begin{lemma}\label{lem:pricing}
There exists a price $p$ such that $BPricingRev_p \geq \frac{1}{2} BRev_0$.
\end{lemma}

\begin{proof}
Let $D_i$ be the value distribution of bidder $i$ for the bundle (which we may think of as just a single item), and let $v_i$ be a sample from $D_i$ denoting bidder $i$'s value. Consider the pricing scheme that first takes a sample $v'_i$ from each $D_i$ and sets reserve $p = \max_i \{v'_i\}$. We show that in expectation, this mechanism achieves revenue at least $BRev_0$.

One way to sample $v_i$ and $v'_i$ is to first take independent samples $\hat{v}_i$ and $\bar{v}_i$ from $D_i$, then with probability $1/2$ assign $v_i := \hat{v}_i$ and $v'_i := \bar{v}_i$, and with probability $1/2$ swap them (call the $v_i$s the ``real'' samples, and the $v'_i$s the ``reserve'' samples). We will show that for all choices of $\hat{v}_i,\bar{v}_i$, the expected (over the randomness of deciding which is $v_i$ and which is $v'_i$) revenue of this pricing scheme is at least $\frac{1}{2} BRev_0$. We define $V_x$ to be the $x^{th}$ largest element of $\cup_i\{v_i,v'_i\}$, $q_x$ to be the probability that the second price auction makes revenue at least $V_x$, and $q'_x$ to be the probability that this pricing scheme makes revenue at least $V_x$. We will show directly that $q'_x \geq q_x/2$ for all $x$, which proves the desired claim.

First, observe that a necessary and sufficient condition for the second price auction to make revenue at least $V_x$, is that at least two of the largest $x$ samples must are ``real.'' This is because the second highest ``real'' sample is exactly the revenue made, and this is at least $V_x$ as long as it is among the largest $x$ samples. Next, observe that a necessary and sufficient condition for the randomized pricing scheme to make revenue at least $V_x$ is that the largest sample is ``real,'' and there is at least one ``reserve'' sample among the largest $x$. This is because if the largest sample is a ``reserve,'' then no one will beat the reserve and therefore the revenue is $0$. If the largest sample is a ``real,'' then certainly someone will beat the reserve, which is exactly the largest ``reserve'' sample. And as long as this sample is among the top $x$, it is at least $V_x$. 

Now, it is clear that $q_1 = q'_1 = 0$, as we cannot have two ``reals'' in the top one sample, and we cannot have both a ``real'' and ``reserve'' in the top one sample either. For all $x > 1$, it is either the case that the top $x$ samples contain both $\hat{v}_i$ and $\bar{v}_i$ for some $i$, or it doesn't. If it does, then the top $x$ samples will always contain a ``reserve'' sample no matter what (because either $\hat{v}_i$ or $\bar{v}_i$ will be one). Therefore, the probability that the top $x$ samples contains a ``reserve'' sample and the top sample is ``real'' is exactly the probability that the top sample is ``real,'' which is $\frac{1}{2}$. As we clearly have $q_x \leq 1$, we get $q'_x = \frac{1}{2} \geq \frac{1}{2}q_x$ in this case. 

If the top $x$ doesn't contain $\hat{v}_i$ and $\bar{v}_i$ for any $i$, then whether each of the top $x$ samples are assigned to ``real'' or ``reserve'' is completely independent. So $q'_x$ is exactly $1/2$ (the probability that the top sample is ``real'') times the probability that at least one of the remaining top $x$ samples is a ``reserve,'' which we'll call $r$. It is clear now that the probability that at least one of the remaining top $x$ samples is a ``real'' is also exactly $r$, and that in order to possibly have two ``real'' samples above $V_x$, we must certainly get at least one from the top $2$ through $x$ samples. So $q_x \leq r$. So in conclusion, we see that $q'_x = r/2$ and $q_x \leq r$, so again we have $q'_x \geq q_x/2$.  


\end{proof}

\begin{corollary}
$BPricingRev \geq BRev/3$. 
\end{corollary}

\begin{proof}
Combining Lemmas~\ref{lem:split} and~\ref{lem:pricing}, there exists a price $q$ such that $BRev_p \leq BPricingRev_p + 2BPricingRev_q \leq 3BPricingRev$. Applying this to the $p$ such that $BRev_p = BRev$ proves the corollary.
\end{proof}

\begin{corollary}
$PPricingRev \geq PRev/3$.
\end{corollary}

\subsection{BUNDLE}
In this section we provide a description of the BUNDLE procedure and prove that it does well when combining schemes that a single bidder is willing to purchase with constant probability. We'll denote each subset in the partition that we start with as $S_1,\ldots,S_k$, their respective prices by $p_1,\ldots,p_k$, and the probability that a single consumer wishes to purchase $S_i$ at price $p_i$ as $q_i \geq c_1$.

We first introduce random variables $V_i$ and $\bar{V}_i$. $V_i = \sum_{j \in S_i} v_j$, and $\bar{V}_i = p_i$, if $V_i \geq p_i$ and $0$ otherwise. In other words, $V_i$ is the value of the consumer for bundle $S_i$. $\bar{V}_i$ is $p_i$ if $S_i$ is purchased and $0$ otherwise. It is clear that $V_i \geq \bar{V}_i$ always. 

Each $\bar{V}_i$ is a $[0,p_i]$ random variable with $\mathbb{E}[\bar{V}_i] = q_ip_i$. So $X = \sum_i \bar{V}_i$ is a $[0,\sum_i p_i]$-random variable with $\mathbb{E}[X] = \sum_i q_i p_i = c\sum_i p_i$ for some $c > c_1$. We can then apply Markov's inequality to the random variable $\sum_i p_i - X$ to get that for any $d < c$:

$$Pr[X \geq d\sum_i p_i] \geq \frac{c-d}{1-d}$$

Which in turn says that:

$$Pr[\sum_i V_i \geq d\sum_i p_i] \geq \frac{c-d}{1-d}$$

So for a fixed $c$, we want to find the $d \in [0,c]$ that maximizes $d\frac{c-d}{1-d}$. Taking derivatives and setting to $0$ we find that this happens at $d = 1-\sqrt{1-c}$. This means that for any $c$, we may set price $(1-\sqrt{1-c})\sum_i p_i$ and sell with probability at least $\frac{c-1 + \sqrt{1-c}}{\sqrt{1-c}}$, making expected revenue at least $(1-\sqrt{1-c}) \frac{c-1+\sqrt{1-c}}{\sqrt{1-c}}\sum_i p_i$. Now, we want to find the choice of $c \in [c_1,1]$ that makes the ratio of this with $c \sum_i p_i$ as small as possible. That is, find the $c \in [c_1,1]$ that minimizes:

$$(1-\sqrt{1-c}) \frac{c-1+\sqrt{1-c}}{c\sqrt{1-c}}$$

Again taking a derivative and setting to $0$, we see that the only local minimum is at $c = 0$, and the derivative is positive on $(0,1)$. So the worst possible ratio when $c \in [c_1,1]$ is attained at $c = c_1$. And we get that the revenue obtained by bundling everything together and setting price $(1-\sqrt{1-c_1})\sum_i p_i$ is at least:

$$(1-\sqrt{1-c_1}) \frac{c_1-1+\sqrt{1-c_1}}{c\sqrt{1-c_1}}\sum_i q_i p_i$$

\subsection{SHATTER}
In this section we provide a description of the SHATTER procedure and prove that it does well when separating a scheme where a single bidder is not willing to purchase, even when the price is reduced by a constant factor, with constant probability. We'll denote the set of items as $S$ and the original (optimal) bundle price as $p$. In Section~\ref{sec:technical} below, we prove a quick technical lemma before getting started with the analysis.


\subsubsection{Technical Lemma}\label{sec:technical}
The point of this lemma is to allow us to remove conditioning in the following section. We let $V$ denote the value of the consumer for the bundle and $v_i$ a single consumer's value for each item $i \in S$.

\begin{lemma}\label{lem:Brendan} Let $p$ be Myerson's reserve and let $A$ be the event that $V \geq p$, and $q = Pr[A]$. Then for all items $i \in S$ and any exponent $j$, we have:

$$Pr[v_i \geq p/2^j | A] \leq 2Pr[v_i \geq p/2^j] + Pr[v_i \geq p/2]/q$$
\end{lemma}

\begin{proof}
By definition, we have:

$$Pr[v_i \geq p/2^j | A] = \frac{Pr[v_i \geq p/2^j \wedge A]}{Pr[A]} = \frac{1}{q}Pr[v_i \geq p/2^j \wedge \sum_{i \in S} v_i \geq p]$$

Also, because all $v_i$ are independent, we have:

\begin{align*}
Pr[v_i \geq p/2^j \wedge \sum_{k \in S} v_k \geq p] &= \int_{p/2^j}^\infty Pr[v_i = x]Pr[\sum_{k \in S -\{i\}} \geq p-x]dx\\
&= \int_{p/2^j}^{p/2} Pr[v_i = x]Pr[\sum_{k \in S-\{i\}} \geq p-x]dx + \int_{p/2}^\infty Pr[v_i = x]Pr[\sum_{k \in S -\{i\}} \geq p-x]dx\\
&\leq \int_{p/2^j}^{p/2} Pr[v_i = x]Pr[\sum_{k \in S} \geq p/2]dx + \int_{p/2}^\infty Pr[v_i = x]dx\\
&\leq Pr[V \geq p/2]Pr[v_i \geq p/2^j] + Pr[v_i \geq p/2]
\end{align*}

Because $p$ is Myerson's reserve, we know that we must have $Pr[V \geq p/2] \leq 2q$. So by the work above, we have:

$$Pr[v_i \geq p/2^j \wedge V \geq p] \leq 2qPr[v_i \geq p/2^j] + Pr[v_i \geq p/2]$$

which concludes the proof of the lemma.
\end{proof}


==> lower-bounds.tex <==
% Example showing Max{Srev,BRev} < PRev/logn for many independent buyers. - Not written (sqrt(n) buyers, each wants a disjoint set of sqrt(n) items iid ER).
% Example showing Max{SRev,BRev} < PRev/logn for one buyer with correlated items. - Not written (partition the items into sets of size sqrt(n). Within partition i, either everything is simultaneously 0, or iid 2^i*ER w.p. 1/2^i).

\section{Lower Bounds}
\mb{this result should eventually be moved to section 5.} 

We next show that there is a setting with many buyers with item valuations that are sampled i.i.d from the same distribution, for which $\PRev(D)$ (and thus also $\max\{\SRev(D), \BRev(D)\}$) provides a poor approximation to $\Rev(D)$.

\begin{proposition}
\label{prop:lb-many-iid}
There exists a setting with $n$ items and many buyers with item valuations that are sampled i.i.d from the same distribution for which
%$\max\{\SRev(D), BRev(D)\}\leq
$\PRev(D)\leq \Rev(D)/\Omega(\log\ n)$.
\end{proposition}
\begin{proof}
Consider a setting with $n$ items and $\sqrt{n}$ buyers with the following value distributions.
For every item $i$ and buyer $j$, the distribution $D_{i,j}$ is sampled i.i.d. as follows.
The value is 0 with probability $1-1/\sqrt{n}$, and with the remaining probability it is sampled from an Equal-Revenue distribution.
To prove the claim we show that $\Rev(D)\in \Omega(n\log\ n)$ while $\PRev(D)\in O(n)$ (actually, as $\SRev\in \Omega(n)$ it holds that $\PRev(D)\in \Theta(n)$).

To see that $\Rev(D)\in \Omega(n\log\ n)$ consider the mechanisms that sequentially go over the $\sqrt{n}$ buyers,
allowing each to pick any set of size $\sqrt{n}$ that are still available, and pay $c(\sqrt{n}\log\ n)$ for some $c>0$ to be determined later.
For each of the $\sqrt{n}/4$ first buyers, with constant probability, the intersection of the set of items for which he has non-zero value and the set of available items has size at least $\sqrt{n}/4$, and thus is willing to pay at least $c_1 (\sqrt{n}\log\ n)$ for some constant $c_1$ (basically, by Lemma 8 of~\cite{HartNisan12}). \mb{need to formally prove this, nit sure this is exactly true. }
Thus the expected revenue from each such buyer is at least $\Omega(\sqrt{n}\log\ n)$ and the total expected revenue is at least $\Omega(n\log\ n)$.

To see that $\PRev(D)\in O(n)$ consider any partition of the items, and denote the size of part $k$ by $s_k$. Note that $\sum_k s_k=n$.






\mb{Proof sketch: Let $S=\{k\ s.t.\ s_k\leq\sqrt{n}\}$ and $L=\{k\ s.t.\ s_k>\sqrt{n}\}$.
For each $k$ such that $k\in S$ it holds that the expected revenue is $O(1)$, and as $|S|\leq n$, the contribution to the expected revenue is $O(n)$.
For each $k$ such that $k\in L$ it holds that with very high probability (MB: will need to use something like Hoeffding's inequality) every buyer value for items in this set is the sum of at most $c s_k /\sqrt{n}$ i.i.d. samples from Equal-Revenue  distributions, for some constant $c>1$. The expected revenue from each such set is at most $c (s_k/\sqrt{n}) \log(c s_k/\sqrt{n})\leq c_1 (s_k/\sqrt{n}) \log(n)$ for some constant $c_1>0$. Summing up over all $k\in L$ gives revenue bounded by
$c_1 \sqrt{n} \log(n)$.
}

\mb{is there an easier proof, or should we just formalize the above?}


\end{proof}
%} % cout

